A Simulation Evaluation Suite for Robust Adaptive Quadcopter Control

Robust adaptive control methods are essential for maintaining quadcopter performance under external disturbances and model uncertainties. However, fragmented evaluations across tasks, simulators, and implementations hinder systematic comparison of these methods. This paper introduces an easy-to-deploy, modular simulation testbed for quadcopter control, built on RotorPy, that enables evaluation under a wide range of disturbances such as wind, payload shifts, rotor faults, and control latency. The framework includes a library of representative adaptive and non-adaptive controllers and provides task-relevant metrics to assess tracking accuracy and robustness. The unified modular environment enables reproducible evaluation across control methods and eliminates redundant reimplementation of components such as disturbance models, trajectory generators, and analysis tools. We illustrate the testbed's versatility through examples spanning multiple disturbance scenarios and trajectory types, including automated stress testing, to demonstrate its utility for systematic analysis. Code is available at https://github.com/Dz298/AdaptiveQuadBench.

==> section/outline.tex <==
\section{Introduction}
\begin{itemize}
    \item \proposefig{figure 1: composite image of quad with wind vector, controller's box plot of tracking error}
    \item Our contribution: 
    \item i) An open-source control library for adaptive control
    \item ii) a standardized testbed for disturbance/uncertainty rejection tasks 
\end{itemize}
\section{Related Work}
\subsection{Adaptive Control for Quadcopters}
\begin{itemize}
    \item intro our selected methods
    \item method targeting on different disturbance/model uncertainty
\end{itemize}
\subsection{Quadcopter Simulators and Benchmarks}
\begin{itemize}
    \item simulator: rotors, airsim, flightmare, rotorpy (lightweight and modular)
    \item open-source benchmark: competition repo? agile flight?  
\end{itemize}
\section{Problem Setup}
\begin{itemize}
    \item \proposefig{system diagram}. Overview of the whole system = Figure~\ref{fig:system-overview}
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/Screenshot from 2025-02-23 14-35-55.png}
    \caption{Overview of our simulation testbed.\todo{user interface notation, include implementation (Random Config, etc)}}
    \label{fig:system-overview}
\end{figure}
\subsection{Quadcopter Dynamics}
\begin{itemize}
    \item model: \proposefig{actuator numbering and x-configuration}
    \item model: params listed, and what model we use? 
    \item dynamics update:xddot 
    \item wdot
    \item note: motor delay, motor noise, air drag
\end{itemize}
\subsection{Controller Design}
\begin{itemize}
    \item reference model
    \item abstraction layer
\end{itemize}
\subsection{Trajectory Tracking}
\begin{itemize}
    \item for large batch eval, we use motion primitives randomization for fast generation while ensuring feasibility
    \item evaluation metrics: RMSE pos, heading error, success rate (if pos larger than 5)
\end{itemize}
\subsection{Disturbance}
Explain each disturbance's implementation
\begin{itemize}
    \item gusty wind
    \item downwash
    \item ground effect (?)
    \item off-center payload
    \item constant force / torque
    \item latency
\end{itemize}
\subsection{Model uncertainty}
\begin{itemize}
    \item individual model uncertainty injection
    \item overall scaling uncertainty (inspired by xadap paper)
\end{itemize}
\subsection{Numerical Setup}
the Table for each experiment type's range. 
\section{Testbed Evaluation}
Should accompanied with python code, with table or figure. 
\subsection{Single Case Eval}

\begin{itemize}
    \item no-uncertainty with all methods's results. Table~\ref{tab:ideal-benchmark} All examples below could generate similar table by switching the experiment type. \todo{controller: all, then do all iterative}
    
    \item wind. we can generate a similar table by using the same command but switching the experiment type. We could also generate a visualization of one single rollout by running command. \todo{python --vis True} 
    Figure x shows a single tracking task of baseline control VS adaptative. Below should all contain visualization code demonstrating different effect, rather than Table (reduce comparison effect)
    \item payload
    \item force/torque
    \item latency
\end{itemize}
\section{When to Fail}
\todo{Not implemented yet}
\begin{itemize}
    \item user can easily increment the magnitude of disturbance until the controller fails to test its robustness boundary. (automatically trigger stop when all trials fail)
    \item python code
    \item example figure: success rate vs wind? individual pos tracking error vs wind? 
\end{itemize}


% \section{Ideal Condition}



% \section{Wind Disturbance}


% \begin{table}[H]
%     \centering
%     \renewcommand{\arraystretch}{1.2} % Adjust row height
%     \begin{tabularx}{\textwidth}{l|cc|XXXX|XXXX|XXXX}
%         \toprule
%         & \multicolumn{2}{c|}{Ideal Condition } 
%         & \multicolumn{4}{c|}{Vertical Wind (e.g., 2 m/s)} 
%         & \multicolumn{4}{c|}{Horizontal Wind (e.g., 2 m/s)}
%         & \multicolumn{4}{c}{Gusty Wind (Dryden Model)} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15}
%         & Pos Error & Heading Error 
%         & Pos Error & Heading Error & Success Rate & Increase over Ideal 
%         & Pos Error & Heading Error & Success Rate & Increase over Ideal
%         & Pos Error & Heading Error & Success Rate & Increase over Ideal \\
%         \midrule
%         Baseline1 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline2 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline3 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline4 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline5 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Performance comparison under different wind conditions, including gusty wind.}
%     \label{tab:wind-benchmark}
% \end{table}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figure/fake_wind.png}
%     \caption{Comparison of success rate with increased wind speed. }
%     \label{fig:wind-robustness}
% \end{figure}


% \clearpage
% \section{Model Uncertainty}

% \begin{table}
%     \centering
%     \renewcommand{\arraystretch}{1.2} % Adjust row height
%     \begin{tabularx}{\textwidth}{l|cc|XXXX|XXXX}
%         \toprule
%         & \multicolumn{2}{c|}{Perfect Model} 
%         & \multicolumn{4}{c|}{Mass ± 30\%} 
%         & \multicolumn{4}{c}{COG Bias ± 30\%, \textbf{ETC}.} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11}
%         & Pos Error & Heading Error 
%         & Pos Error & Heading Error & Success Rate & Increase over Ideal 
%         & Pos Error & Heading Error & Success Rate & Increase over Ideal \\
%         \midrule
%         Baseline1 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline2 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline3 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline4 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         Baseline5 & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
%         \bottomrule
%     \end{tabularx}
%     \caption{Performance comparison under different model uncertainties over individual parameters (mass, COG, motor constant, etc).}
%     \label{tab:model-uncertainty}
% \end{table}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figure/fake_model.png}
%     \caption{Comparison of success rate with increased model uncertainty (over all components). }
%     \label{fig:model-robustness}
% \end{figure}







==> section/review.tex <==
% Reviewer 1
This paper addresses a critical gap in the evaluation and benchmarking
of quadcopter control strategies under various disturbances and
uncertainties. The authors propose a modular, open-source simulation
framework built on RotorPy, which streamlines the process of
systematically assessing different control algorithmsóparticularly
robust adaptive controllersóacross diverse disturbance scenarios.

While the overview is thorough, the paper could benefit from more
detailed descriptions of the underlying algorithms, especially
regarding how adaptive controllers are integrated with the simulation
environment and how disturbances are parameterized and injected
dynamically.

The paper mainly introduces the framework. Including preliminary
results or case studies demonstrating its effectiveness and validation
against hardware experiments would strengthen the contribution and
illustrate practical utility.

% Reviewer 2
The paper proposes a quadcopter control toolbox in python with several
adaptive control methods benchmark under a unified framework.

The paper is well written, well structured, and easy to read.

However I have some serious concerns about the novelty, and most
importantly, the relevance of the benchmark.

First, while it is nice that we can have a well-organized, cleanly
coded suite of adaptive control algorithms to quickly test out, these
methods were published in other works, and for classic model-based
control algorithms the coding part is not the hard part, but the
analyses and mathematical proof to establish the convergence and
gauranteeing of control objectives. So what the authors are doing here
is mainly just "clerical work", which I would also think it might be
better to let students try out themselves.

Second, the toolbox is lightweight, but it also comes with the issue of
lacking potential for application beyond the niche of adaptive control,
for quadcopter. I look at the list of the methods included in the
toolbox, there seems to be only one learning-based control methods and
the rest are classic ones. In my opinion learning-based control is the
future, and it's being extensively explored in data-driven, end-to-end,
or reinforcement learning approaches. We are really in need of more
educational and instructional examples for reinforcement learning on
advance framework such as Isaac Sim or Mujoco, not a library appears to
be a simple documentation of a bygone era.

I also note that Professor Peter Corke's longstanding robotics toolbox
has also had python version at
https://petercorke.github.io/robotics-toolbox-python/intro.html

So maybe the authors can convert this into an extension of his toolbox
and submit to the RAS CASE conference.

Corke, Peter, and Jesse Haviland. "Not your grandmother’s toolbox–the
robotics toolbox reinvented for python." In 2021 IEEE international
conference on robotics and automation (ICRA), pp. 11357-11363. IEEE,
2021.

% Reviewer 3
Summary:
The paper presents an open source benchmark written in Python, based on
the RotorPy simulator, which supports several realistic aerodynamics
effect, to develop and test robust multicopter controllers. The
benchmark suite come with several state-of-the-art controller
implementations (mpc, geometric, model-free, indi, etc) and API to
generate simple trajectories as well as external (wind) and internal
(model-mismatch) distrurbances. Comparisons, repeated trials, and
visualization are also already scripted in the evaluation suite.
The usefulness of the tool is demonstrated through several examples
showing how the suite can help investigate the breaking points of
different controller w.r.t. do different disturbances.

Strengths:
The paper is well-written (a few typos, presentation mishaps a listed
below), very well-structured and easy to follow.
The motivation is clearly stated, the implementation leverages
state-of-the-art tools and is accompanied by an open-source
implementation with clear connections between the source code and the
experiments/plots in the paper.




%%%%%%% Done %%%%%%%%%%%%%%%
Detailed comments, typos, and requests for clarification:

- the motivation for using an aerodynamic model inspired by [17] and
not the default RotorPy is unclear: what is the trade-off? what is
better modeled by one or the other? are there computational
considerations to make? it would also be mention the RotorPy
aerodynamic effects that are being considered at the beginning of the
section, before the in-depth modeling, rather than at the end.
- One caveat, if you list the acados dependency as optional, then please
provide examples in the readme that do not require it: I tried to copy
and paste a few of them an always got thrown an acados_template error.
I guess run_eval always imports and MPC controller with acados
dependencies, so either make the import conditionals or make acados a
required dependency and provide installation instructions direclty in
the readme (plus cross-link).
- on page 1, left column, several \cite{} commands are not spaced from
the text, use ~\cite{}
- In the caption of Figure 4 possibly explain why the controllers
deviate from the desired trajectory even before the payload is attached
- The figures are seemingly not referenced introduced in order in the
text (e.g Figure 4, then 7 then 6), should the Figure 7 reference be to
Figure 5 instead?
- I think there is a bit of an obvious omission in the reference list:
https://arxiv.org/abs/2109.06325 seems to have a very similar
rationale; I would argue that the proposed submission has a lot of
merit because it has a more thorough focus on quadcopter dynamics
modelling (while https://github.com/utiasDSL/safe-control-gym uses
simple CasADi dynamics and/or a general purpose physics engine in
Bullet) and intoduce other state-of-the-art controllers like INDI, but
the attemp to standardize disturbances for robust quadrotor control is
not novel and it should be stated

